Generative Adversarial Networks for MR-CT Deformable Image Registration

Deformable Image Registration (DIR) of MR and CT images is one of the most challenging registration task, due to the inherent structural differences of the modalities and the missing dense ground truth. Recently cycle Generative Adversarial Networks (cycle-GANs) have been used to learn the intensity relationship between these 2 modalities for unpaired brain data. Yet its usefulness for DIR was not assessed. In this study we evaluate the DIR performance for thoracic and abdominal organs after synthesis by cycle-GAN. We show that geometric changes, which differentiate the two populations (e.g. inhale vs. exhale), are readily synthesized as well. This causes substantial problems for any application which relies on spatial correspondences being preserved between the real and the synthesized image (e.g. plan, segmentation, landmark propagation). To alleviate this problem, we investigated reducing the spatial information provided to the discriminator by decreasing the size of its receptive fields. Image synthesis was learned from 17 unpaired subjects per modality. Registration performance was evaluated with respect to manual segmentations of 11 structures for 3 subjects from the VISERAL challenge. State-of-the-art DIR methods based on Normalized Mutual Information (NMI), Modality Independent Neighborhood Descriptor (MIND) and their novel combination achieved a mean segmentation overlap ratio of 76.7, 67.7, 76.9%, respectively. This dropped to 69.1% or less when registering images synthesized by cycle-GAN based on local correlation, due to the poor performance on the thoracic region, where large lung volume changes were synthesized. Performance for the abdominal region was similar to that of CT-MRI NMI registration (77.4 vs. 78.8%) when using 3D synthesizing MRIs (12 slices) and medium sized receptive fields for the discriminator.

==> literatureReview.tex <==
Why MR-CT image registration?
\begin{itemize}
\item to fuse complementary information (density for radiation therapy, bones from CT and soft-tissue from MRI)
\item transfer of segmentations, treatment plans over time
\item image registration: spatial correpondences between same subjects
\end{itemize}
GAN and image registration
\begin{itemize}
\item GAN: model to create {\bf plausible} images from a population, but not necessarily realistic, exact synthesized image from a given image for unpaired data
\item why GAN for image registration? Hypothesis: that unsupervised GAN image synthesis eases/improves image registration, by allowing a simpler image similarity measure
\item unpaired data attractive for CT-MRI deformable image registration as hard to know gold standard deformations
\item use GANs on unpaired data to learn plausible image synthesis between CT and MRI for particular anatomical regions. Constrain synthesis on paired data + image deformable registration
\item independent synthesis and registration vs. pretrained sythesis + combined end-to-end synthesis + deformable registration
\end{itemize}

Issues
\begin{itemize}
\item 3D (RGB) consistency vs. 2D, generally not shown; nobody using 3D
\item issue: modalities acquired in different anatomical configurations (arms up/down, end-exhale vs. end-inhale), GAN will also learned to undo these to be realistic, however this can affect image correspondence
\item intensity conversion to create other modality also to compensate for changes in anatomical location (i.e. adding structures like arms or changing lungs size)
\item GANs change image intensities to also compensate for motion changes. The associated segmentations are then not correct anymore, and subsequent image registration fails. Hence, their use for cardiac segmentation needed incorporation of the segmentation masks~\cite{chartsias2017adversarial}. Here we propose to train motion-aware cycle-GANs, which have two main options to generate realistic images: (a) intensity changes and (b) local spatial transformations. The trade-off between these two options is regulated by the cost function. We want to simplest model, which can create realistic images. Formulating the problem as a regression problem, which incorporates image registration end-to-end, instead of a population-wide classification problem has the advantage of providing as a by product a population appearance and motion model.  This is similar to conventional statistical shape and appearance models (SSAM), only that the model is encodes as a deep neural network. We show the advantage of using DNNs over SSAMs ....  
\item cycle-GAN vs. deep SSAM! deep SSAM formulated as ...
\item cycle-GAN generator including a local spatial transformer, transformation cost includes NMI or edge cost between image modalities? must be cheaper to move an edge than to remove and create an edge for fakeImage. Smooth motion and local intensity change consistency (patch-wise consistent)?
\item unpaired really better than registered+paired for scenarios where motion is contained within the population and for image registration?
\end{itemize}



\subsection{Paired data}

\begin{itemize}
\item \cite{van2015cross}: van2015cross, Cross-Domain Synthesis of Medical Images Using Efficient Location-Sensitive Deep Network
\begin{itemize}
\item T1-T2, brain MRIs, 
\item rigidly aligned (rough alignment)
\item leave-one-out cross validation
\item location-sensitive deep network (LSDN) e.g. 30-400-40-1 with
input: 27 intensity values of 3$^3$ ROI, 3 position values (x,y,z) and output: intensity value of center voxel
\item LSDN models hidden nodes as products of intensity features
and spatial responses
\end{itemize}

\item \cite{nie2017medical}: nie2017medical, paired data
\begin{itemize}
\item addresses misalignment by incorporating an image-wise loss
\item contains a voxel-wise
loss component requiring a training set of paired MR and CT volumes
\end{itemize}

\item \cite{zhou2017generating}: zhou2017generating, virtual CT from MRI using fully convolutional neural networks (Master thesis)
\begin{itemize}
\item 17 non-rigidly registered (B-Spline, elastix, manual segmentation of disturbing areas (air, Brachy seeds)) prostate images
\item fully connected CNN, patches of 24$^3$ voxels, step size 4
\item investigates different loss functions (SSIM instead of L2, L1) for regression problem
\end{itemize}


\item \cite{yang2017fast}: yang2017fast, Fast predictive multimodal image registration (ISBI18)
\begin{itemize}
\item abstract
\begin{itemize}
\item deep encoder-decoder architecture for image
deformation prediction from multimodal images
\item image-patch-based deep network that jointly (i)
learns an image similarity measure and (ii) the relationship
between image patches and deformation parameters
\item focus on the Large Deformation Diffeomorphic
Metric Mapping (LDDMM) registration model
\item predicting
the initial momentum of the shooting formulation of
LDDMM, we preserve its mathematical properties and drastically
reduce the computation time, compared to optimization based
approaches
\item Bayesian probabilistic
version of the network that allows evaluation of registration
uncertainty via sampling of the network at test time
\item3D brain MRI dataset using both
T1- and T2-weighted images
\item method generates accurate predictions and that learning
the similarity measure leads to more consistent registrations
than relying on generic multimodal image similarity measures,
such as mutual information
\item approach is an order
of magnitude faster than optimization-based LDDMM
\end{itemize}
\item method
\begin{itemize}
\item encoder-decoder
network, where two encoders compute features from the moving/
target image patches (15$^3$) independently
\item learned features concatenated and sent to
three decoders to generate one initial momentum patch
\item use convolutional layers with a stride of
2 and deconvolution layers as surrogates for pooling and
unpooling layers
\item For training, we use the
L1 norm as our similarity criterion
\item during testing: sliding window approach,
predicting the momentum patch-by-patch, followed by averaging momenta in overlap region
\item for uncertainty: Bayesian network via dropout (prob. 0.3) and during testing several predictions. Mean used as result, variance of predictions as uncertainty
\item patch pruning: use large stride (14) and ignore background patches
\end{itemize}
\item experiment
\begin{itemize}
\item IBIS 3D Autism Brain image
dataset, containing 375 T1w/T1w brain images (229 $\times$
193 $\times$ 193) of 2 years subject with pediatric disease
\item all images are registered affinely to the ICBM 152 atlas
\item 359 images for training, 16 images for testing
\item For training, we randomly select 359 T1w-T1w image pairs and perform LDDMM registration with SSD as image similarity measure
\item then network is trained to predict the momenta generated
from the T1w-T1w registrations using their corresponding
T1w and T2w images. REQUIRES CORRESPONDENCE between T1w and T2w!!!!
\item evaluation based on `gold-standard' of LDDMM registration of T1w-T1w registration (BIASED!)
\item NOT compared to LDDMM with MI, or on independent measures (landmarks, overlaps)!
\end{itemize}
\end{itemize}

\end{itemize}

\subsection{Unpaired data}
\begin{itemize}

\item \cite{liu2016coupled}: liu2016coupled, Coupled Generative Adversarial Networks
\begin{itemize}
\item for learning a joint
distribution of multi-domain images without any tuple of corresponding images
\item one GAN per domain (e.g. image, depth map), GANs sharing weights (some first layers of generators, some last layers of discriminator)
\end{itemize}

\item \cite{vemulapalli2015unsupervised}: vemulapalli2015unsupervised, Unsupervised Cross-modal Synthesis of Subject-specific Scans
\begin{itemize}
\item T1/T2 brain MRI, 19 subjects
\item without alignment
\item Given a source modality image of a subject, we first generate multiple target modality candidate values for each voxel
independently using cross-modal nearest neighbor search.
\item Then, we select the best candidate values jointly for all
the voxels by simultaneously maximizing a global mutual
information cost function (mutual information) and a local spatial consistency
cost function (neighbours should have similar cadidates)
\item Finally, we use coupled sparse representation
for further refinement of synthesized images (dictionary of patches, SVD)
\end{itemize}

\item \cite{zhu2017unpaired}: zhu2017unpaired, cycle GAN, unpaired data
\begin{itemize}
\item proposal of cycle GAN
\item horse/zebra etc.
\item limitations visible (e.g. zebra strips on fence, rider etc.)
\end{itemize}

\item \cite{chartsias2017adversarial}: chartsias2017adversarial, unpaired cardiac data, with segmentation masks
\begin{itemize}
\item CycleGAN, unpaired images
\item synthesising cardiac MR images from CT images, using a
dataset of MR and CT images coming from different patients
\item abstract
\begin{itemize}
\item leveraging our synthetic data to achieve improved results in segmentation
\item training on both real and synthetic data increases accuracy by 15\%
compared to real data
\item synthetic data is of sufficient
quality to be used alone to train a segmentation neural network, that
achieves 95\% of the accuracy of the same model trained on real data
\end{itemize}
\item incorporates ViewAlignment
\begin{itemize}
\item make the CT and MR image sets broadly similar
in terms of structure
\item to make layout of images
(e.g. position, size of anatomy) not informative as to
dataset from which image came
\item otherwise the discriminator may learn
to differentiate between real and synthetic data by attending to structural differences, rather than intensity statistics
\item alignment only needs to
be approximate;
use multiple labels (supervised!), to approximate
affine transformation to align
CT volume with MR volume
\item after crude alignment,
any points in new volume that correspond to points outside of
the original volume are set to 0
\end{itemize}
\item $I_{CT}$ with
its segmentation mask $S_{CT}$ is mapped to synthetic MR $G_{MR}(I_{CT})$ and synthetic MR mask $G_{MR}(S_{CT})$ by a generator network $G_{MR}$.
Discriminator $D_{MR}$ then tries to discriminate real
from synthetic MR. The CT and Mask are also reconstructed form the synthetic MR by generator network $G_{CT}$. The generator learns both by trying to fool the discriminator,
and by minimising the discrepancy between the real CT and its reconstruction.
\end{itemize}

\item \cite{wolterink2017deep}: wolterink2017deep, MRI to CT sythesis via cycle GAN on unpaired brain data.
\begin{itemize}
\item 24 patients (18 training, 6 test), brain CT, MR images same day; radiotherapy; 183 $\times$ 288 $\times$ 288 voxels
\item rigidly aligned based on MI to allow comparison
\item evaluation: mean absolute error (MAE) and peak SNR were computed within a head region mask
\item 2D sagittal slices (183 slices), each image was padded to 286 $\times$ 286 pixels and sub-images of 256 $\times$ 256 pixels were randomly cropped during training
\item trained using Adam for 100 epochs with a fixed learning rate of 0.0002, and 100 epochs in which the
learning rate was linearly reduced to zero
\item random slices + cropping from same aligned patient, so discriminator might remember same anatomy (not completely unpaired)
\item Model training took 52 hours on a
single NVIDIA Titan X GPU. MR to CT synthesis with a trained model took
around 10 seconds.
\item cycle GAN
\begin{itemize}
\item generators: 2D fully convolutional networks with two strided convolution layers
\item 9 residual blocks and two fractionally strided convolution layers, based on the architecture used in \cite{zhu2017unpaired}
\item CNN takes input images of size 256 $\times$ 256 pixels
\item discriminators:  fully convolutional architecture to classify overlapping 70 $\times$ 70 image patches as real or fake
\end{itemize}
\item loss: $L_{CT}$+$L_{MR}$+$\lambda L_{cycle}$\\
discriminator loss: \\
$L_{CT}=(1 - D_{CT}(I_{CT}))^2 + D_{CT}(G_{CT}(I_{MR} ))^2$\\
$L_{MR}=(1 - D_{MR}(I_{MR}))^2 + D_{MR}(G_{MR}(I_{CT} ))^2$\\
generator cycle loss: \\
$L_{cycle}=||G_{CT}(G_{MR}(I_{CT}))-I_{CT}||_{1}$ + 
$||G_{MR}(G_{CT}(I_{MR}))-I_{MR}||_{1}$
\item paired data
\begin{itemize}
\item an additional synthesis CNN with the same architecture as $G_{CT}$ was trained using paired MR and CT image slices
\item used the implementation of \cite{isola2016image}
which, like \cite{nie2017medical}, combines voxel-wise loss with adversarial feedback from a discriminator network
\item higher MSE (89 vs. 74 HU) for paired training; 
\item results with unpaired data looked more realistic,
contained less artifacts and contained less blurring than those obtained from paired data
\item why? blurry? due to slight misalignments? 
\end{itemize}
\end{itemize}


\item \cite{costa2017end}: costa2017end, End-to-end Adversarial Retinal Image Synthesis
\begin{itemize}
\item adversarial autoencoder trained to reconstruct retinal vessel maps (hidden space
\item Generative
Adversarial Network trained to generate color retinal images out of vessel maps
\item Discriminator to differentiate synthetic and real pairs of vessel maps + color retinal images
\item generating 
retinal images with their corresponding vessel
networks, by sampling from a simple probability distribution (latent space of autoencoder)
\item We show that the
learned latent space contains a well-defined semantic structure,
implying that we can perform calculations in the space of retinal
images, e.g., smoothly interpolating new data points between two
retinal images
\item synthesized images are substantially different from those in
the training set (visual inspection of closest training example measured by MI of retinal vessel maps), while being also anatomically consistent and
displaying a reasonable visual quality.
\end{itemize}

\item \cite{calimeri2017biomedical}: calimeri2017biomedical, GANs to the automatic generation of artificial Magnetic Resonance Images (MRI) of slices of the human brain
\begin{itemize}
\item
\end{itemize}


\item \cite{huo2017adversarial}: huo2017adversarial, Adversarial Synthesis Learning Enables Segmentation Without Target Modality Ground Truth (ISBI18)
\begin{itemize}
\item abstract
\begin{itemize}
\item Previously~\cite{chartsias2017adversarial}, two stage methods have been proposed
to use cycle generative adversarial networks (CycleGAN) to
synthesize training images for a target modality. Then, these
efforts trained a segmentation network independently using
synthetic images. 
\item However, these two independent stages did
not use the complementary information between synthesis
and segmentation. 
\item Herein, we proposed a novel end-to-end
synthesis and segmentation network (EssNet) to achieve the
unpaired MRI to CT image synthesis and CT splenomegaly
segmentation simultaneously without using manual labels on
CT
\item EssNet achieved significantly higher
median Dice similarity coefficient (0.9188) than the two
stages strategy (0.8801), and NOT SIGNIFICANT higher than canonical
multi-atlas segmentation (0.9125) and ResNet method
(0.9107), which used the CT manual labels
\end{itemize}
\item experiment
\begin{itemize}
\item 60 whole abdomen MRI T2w scans, 19 whole
abdomen CT with splenomegaly spleen (abnormally large spleen)
\item 6 labels (spleen, left kidney, right kidney, liver, stomach and
body) were manually delineated for each MRI, while one
label (spleen) was manually traced for each CT scan
\item 75 whole abdomen CT scans with normal spleens
were used to train a baseline DCNN method
\end{itemize}
\item method
\begin{itemize}
\item cycleGAN and additionally: manual segmentation input $S_{MR}$ for $I_{MR}$, prediction of segmentation of CT via segmentation network $S$, discrimination of real or fake CT segmentation
\item The segmentation
network $S_{CT}$ was concatenated after $G_{CT}$ directly as an additional
forward branch (9 block ResNet used, identically to $G_{CT}$)
\item additional segmentation loss function ($L_{CT}$+$L_{MR}$+$\lambda_{cycle} L_{cycle}+\lambda_{seg} L_{seg}$):\\
$L_{seg}(S_{CT},G_{CT},I_{MR})$ $=$ $-\sum_i m_i log(S_{CT}(G_{CT}(I_{MR_i})))$
where $m$ is the manual labels for image $I_{MR}$, $i$ is the index
of a pixel (pixel-wise as fakeCT and MR should be in correspondence, hence fakeCTsegm and MRsegm as well); $\lambda_{cycle}=10, \lambda_{seg}=1$
\item during testing, only $S_{CT}$ used (not fakeCT) to produce segmentation from real $I_{CT}$
\end{itemize}
\item this approach should avoid compensation for motion by intensity conversion, as constrained by manual segmentations (only works if there is not a large motion between images as otherwise dicriminator can easily differentiate fake from real images) - can this be done without MANUAL segmentations? supervoxels? edges? MI? but then impose structures which may be different in the two modalities. Need to incorporate displacements as another way to compensate for differences
\item likely not to work with large systematic motion between modalities
\item could this be used for predicting landmark locations in other modality instead of segmentation?
\end{itemize}

\end{itemize}

\subsection{Other related work}
\begin{itemize}
\item \cite{theis2015note}: theis2015note, a note on evaluation of GANs
\begin{itemize}
\item show that three of the currently most commonly
used criteria—average log-likelihood, Parzen window estimates, and visual
fidelity of samples—are largely independent of each other when the data is
high-dimensional
\item generative
models need to be evaluated directly with respect to the application(s) they were
intended for
\item  demonstrating that Parzen window
estimates should generally be avoided
\end{itemize}

\item \cite{worrall2017interpretable}: worrall2017interpretable, Interpretable Transformations with Encoder-Decoder Networks
\begin{itemize}
\item want to disentangle confounding factors, such as pose, appearance,
and illumination, from object identity
\item custom feature transform layer (incorporate spatial transformer), acting on the hidden representations
\end{itemize}

\item \cite{tran2017disentangled}: tran2017disentangled, Disentangled representation learning GAN for pose-invariant face recognition
\begin{itemize}
\item proposes Disentangled
Representation learning-Generative Adversarial
Network (DR-GAN) 
\item input: face image $\mathbf{x}$ with identity label $y^d$ and pose label $y^p$, target pose code $\mathbf{c}$, random noise $\mathbf{z}$ (SUPERVISED!)
\item generator $G$
\begin{itemize}
\item to generate same face with target pose that fools discriminator $D$
\item $G_{enc}$: learns
mapping from image  $\mathbf{x}$ to feature representation $f(\mathbf{x})$
\item $G_{dec}$: generates face image $\mathbf{\hat{x}}$ with target rotation from $f(\mathbf{x})$, $\mathbf{c}$, $\mathbf{z}$
\end{itemize}
\item discriminator $D$ 
\begin{itemize}
\item trained to distinguish
real vs. synthetic images, and also predict the identity
and pose of a face
\item multi-task CNN consisting of two parts: $D =
[D^d,D^p]$
\item $D^d \in R^{N^{d+1}}$ is for identity classification with
$N^d$ as the total number of subjects in the training set and the
additional dimension is for the fake class
\item $D^p \in R^{N^p}$ is for
pose classification with $N^p$ as the total number of discrete
poses for real image $\mathbf{x}$
\end{itemize}
\item DR-GAN can
take one or multiple images as the input, and generate one
unified representation along with an arbitrary number of
synthetic images
\end{itemize}

\item \cite{baumgartner2017visual}: baumgartner2017visual, WGAN to then get voxel-wise disease classification map
\begin{itemize}
\item Wasserstein GAN used to learn additive mapping between MCI and Alzheimer's Disease from unpaired brain data to get voxel-wise disease classification map
\item preprocessing: rigid alignment to MNI space, bias field corrected, skull stripping, resampled to 1.3mm$^3$ resolution, rescaled to [-1,1] intensity
\item evaluated based on NCC between predicted and observed change (latter after rigid image registration) for paired data (excluding different field strength), very low NCC (0.24) for real data (high for synthetic experiment: 0.94)
\item novel: no need for image registration as edges are `moved' by image synthesis
\item novel: processing of large 3D data
\end{itemize}
\end{itemize}


